Quadratic transformations of Macdonald and Koornwinder polynomials

When one expands a Schur function in terms of the irreducible characters of the symplectic (or orthogonal) group, the coefficient of the trivial character is 0 unless the indexing partition has an appropriate form. A number of q-analogues of this fact were conjectured in math.QA/0112035; the present paper proves most of those conjectures, as well as some new identities suggested by the proof technique. The proof involves showing that a nonsymmetric version of the relevant integral is annihilated by a suitable ideal of the affine Hecke algebra, and that any such annihilated functional satisfies the desired vanishing property. This does not, however, give rise to vanishing identities for the standard nonsymmetric Macdonald and Koornwinder polynomials; we discuss the required modification to these polynomials to support such results.

==> notes.tex <==
\section{Internal notes}

For our reference, I'm recording here the various vanishing results, and
associated ideals.

\subsection{Macdonald polynomial results: $\tilde{S}_{2n}$}

Each ideal comes from a subgroup of the braid group, and is generated by
elements
\[
\sigma-\chi(\sigma)
\]
where $\chi$ is the character of $B$ given by its action on the constant
polynomials.

\subsubsection{Ideal 1}
\[
S = \langle T_0,T_n,T_iT_{2n-i}^{-1}\rangle
\]
Chambers are such that $r$ and $r^\omega$ have the same sign, where
$\omega$ is the longest element of $S_n$, and $r$ is a root such that
$r+r^\omega\ne 0$.  Invariant functionals ($L(\sigma f)=0$, $\sigma\in S$)
vanish on $E^C_\lambda$ unless $\lambda_i=\lambda_{2n+1-i}$, $1\le i\le n$.

Take
\[
L(p)
=
\int p(z_1,z_2,\dots z_n,1/z_n,\dots 1/z_2,1/z_1)
\prod_{1\le i\le n} \frac{(z_i^2,q z_i^{-2};q)}{(t z_i^2,q t z_i^{-2};q)}
\prod_{1\le i<j\le n} \frac{(z_i z_j^{\pm 1},q z_i^{-1} z_j^{\pm 1};q)}
                           {(t z_i z_j^{\pm 1},qt z_i^{-1} z_j^{\pm 1};q)}
dT
\]
% CHECKED compatible with conventions.tex

Implies
\[
\label{Sn1}
\int
P_\lambda(\dots z_i^{\pm 1}\dots;q,t)
\prod_{1\le i\le n} \frac{(z_i^{\pm 2};q)}{(t z_i^{\pm 2};q)}
\prod_{1\le i<j\le n} \frac{(z_i^{\pm 1} z_j^{\pm 1};q)}
                           {(t z_i^{\pm 1} z_j^{\pm 1};q)}
dT
=
0
\]
unless $\lambda=\mu^2$.

Conjugate consists of two identities, each involving a sum of two integrals (see
\cite{bcpoly}).

\subsubsection{Ideal 2}
\[
S = \langle T_{2i-1},T_{2i}T_{2i-1}T_{2i+1}^{-1}T_{2i}^{-1},
                     T_{2i}^{-1}T_{2i-1}T_{2i+1}^{-1}T_{2i},\shift^2\rangle
\]
\comment{T vs U, ideals redo}
Chambers are such that $r$ and $r^\iota$ have opposite signs, where
$\iota(2i-1)=2i$, $\iota(2i)=2i-1$.  $I$-invariant functionals vanish on
$E^C_\lambda$ unless $\lambda_{2i-1}+\lambda_{2i}=0$, $1\le i\le n$.

Functional 1:
\[
L(p)
=
\int p(z_1,-z_1,z_2,-z_2,\dots z_n,-z_n)
\prod_{1\le i<j\le n} \frac{(z_i^2/z_j^2,q^2 z_j^2/z_i^2;q^2)}
                           {(t^2 z_i^2/z_j^2,q^2 t^2 z_j^2/z_i^2;q^2)}
dT
\]
% CHECKED

Implies
for partitions $\mu, \nu$ that
\[
\int
P^{(2n)}_{\mu\bar\nu}(\dots \pm \sqrt{z_i}\dots;q,t)
\prod_{1\le i\le n} \frac{((z_i/z_j)^{\pm 1};q^2)}{(t^2 (z_i/z_j)^{\pm 1};q^2)}
dT
=
\int
P^{(2n)}_{\mu\bar\nu}(\dots \pm \sqrt{z_i}\dots;q,t)
\widetilde \Delta_S^{(n)}(q^2, t^2)
dT
=
0
\]
unless $\mu=\nu$. 
Note that this is well-defined because
$P^{(2n)}_{\mu\bar\nu}(\dots \pm \sqrt{z_i}\dots;q,t)$
is invariant under $\sqrt{z_i} \mapsto - \sqrt{z_i}$
and it is therefore in $\C(q,t)[{z_1}^{\pm 1},\ldots, {z_n}^{\pm 1} ].$
 In symmetric function terms:
\[
[P_{m^n}(;q^2,t^2)] P_\lambda([2p_{k/2}];q,t)
=
0
\]
unless $\lambda=(2m)^{2n}-\lambda$.  Self-dual.

Functional 2:
\[
L(p)
=
\int
p(z_1,t z_1,z_2,t z_2,\dots z_n,t z_n)
\prod_{1\le i<j\le n} \frac{(z_i/z_j,q z_j/z_i;q)}
                           {(t^2 z_i/z_j,q t^2 z_j/z_i;q)}
dT
=
\int
p(z_1,t z_1,z_2,t z_2,\dots z_n,t z_n)
\widetilde \Delta_S^{(n)}(q, t^2)
dT
\]
% CHECKED

Implies
\[
\int
P^{(2n)}_{\mu\bar\nu}(\dots t^{\pm 1/2}z_i\dots;q,t)
\prod_{1\le i<j\le n} \frac{((z_i/z_j)^{\pm 1};q)}
                           {(t^2 (z_i/z_j)^{\pm 1};q)}
dT
=
0
\]
unless $\mu=\nu$.  In symmetric function terms:
\[
[P_{m^n}(;q,t^2)] P_\lambda([p_k (t^{k/2}+t^{-k/2})];q,t)
=
0
\]
unless $\lambda=m^{2n}-\lambda$.  Odd $m$ uses rationality in $t^n$ of
dual result for $P_{\mu\bar\nu}$:
\[
[P_{m^n}(;q^2,t)] P_\lambda(;q,t)
=
0
\]
unless $\lambda=(2m)^n-\lambda$.  Nonzero values appear nice, but Pieri
trick fails.

\subsubsection{Ideal 3}
\[
S = \langle T_i T_{i+n}^{-1},\Delta\rangle
\]
Chambers are such that $r$ and $r^\iota$ have opposite signs, where
$\iota(i)=i+n$, $\iota(i+n)=\iota(i)$.  $I$-invariant functionals vanish
on $E^C_\lambda$ unless $\lambda_i+\lambda_{i+n}=0$.

Functional:
\[
L(p)
=
\int
p(q^{1/2} z_1, q^{1/2} z_2,\dots q^{1/2} z_n,
  z_1,z_2,\dots z_n)
\prod_{1\le i<j\le n} \frac{(z_i/z_j,q^{1/2} z_j/z_i;q^{1/2})}
                           {(t z_i/z_j,q^{1/2} t z_j/z_i;q^{1/2})}
=
\int
p(q^{1/2} z_1, q^{1/2} z_2,\dots q^{1/2} z_n,
  z_1,z_2,\dots z_n)
\widetilde \Delta_S^{(n)}(\sqrt q, t)
\]
% CHECKED

Implies ($q\mapsto q^2$)
\[
\int
P^{(2n)}_{\mu\bar\nu}(\dots q^{\pm 1/2}z_i\dots;q^2,t)
\prod_{1\le i<j\le n} \frac{((z_i/z_j)^{\pm 1};q)}
                           {(t (z_i/z_j)^{\pm 1};q)}
dT
=
0
\]
unless $\mu=\nu$.  In symmetric function terms:
\[
[P_{m^n}(;q,t)] P_\lambda([p_k (q^{k/2}+q^{-k/2})];q^2,t)
=
0
\]
unless $\lambda=m^{2n}-\lambda$.  Dual:
\[
[P_{m^n}(;q,t)] P_\lambda(;q,t^2)
\]
unless $\lambda=(2m)^n-\lambda$.  Nonzero values appear nice, but Pieri
trick fails.

\subsection{Koornwinder polynomial results: $\widetilde{C}_{2n}$}

\subsubsection{Ideal 1}
\[
S = \langle
T_{2i-1},T_{2i}^{\pm 1}T_{2i-1}T_{2i+1}^{-1}T_{2i}^{\mp 1},
T_0^{\pm 1} T_1 T_0^{\mp 1},
T_{2n}^{\pm 1} T_{2n-1} T_{2n}^{\mp 1}
\rangle
\]

Functional 1:
\[
L(p)
=
\int
p(z_1^{1/2},-z_1^{1/2},z_2^{1/2},-z_2^{1/2},\dots z_n^{1/2},-z_n^{1/2})
%%\dots
\Delta_C^{(n)}(a^2, -t, c^2, -qt; q^2, t^2)
\]
\comment{
($b=-a$, $d=-c$; density is nonsymmetric Koornwinder with
$q'=q^2,t'=t^2,a'=a^2,b'=-t,c'=c^2,d'=-qt$)}
In symmetric function terms,
\[
I_K(\tilde{K}_\lambda([2p_{k/2}];q,t,T;a,-a,b,-b);q^2,t^2,T;-t,-qt,a^2,b^2)
=
0
\]
unless $\lambda=\mu^2$.  Dually,
\[
I_K(\tilde{K}_\lambda([2p_{k/2}];q,t,T;a,-a,b,-b);q^2,t^2,T;-1,-t,a^2,b^2)
=
0
\]
unless $\lambda=2\mu$.  (For $T=t^{2n}$ and $T=t^{2n+1}$, this simplifies
as an integral (only one each, though).)
The nonzero values are FOO. \comment{foo!!}

Functional 2:
\[
L(p)
=
\int
p(t^{-1/2} z_1,t^{1/2} z_1,t^{-1/2} z_2,t^{1/2} z_2,\dots
t^{-1/2} z_n,t^{1/2} z_n)
\Delta_C^{(n)}(t^{1/2}a, t^{1/2}b, t^{1/2}c, t^{1/2}d; q, t^2)
%%\dots
\]
$q'=q,t'=t^2,a'=t^{1/2}a,b'=t^{1/2}b,c'=t^{1/2}c,d'=t^{1/2}d$

In symmetric function terms,
\[
\label{IK}
I_K(\tilde{K}_\lambda([p_k(t^{k/2}+t^{-k/2})];q,t,T;a,b,c,d);
    q,t^2,T;t^{1/2}a,t^{1/2}b,t^{1/2}c,t^{1/2}d)
=
0
\]
unless $\lambda=\mu^2$.  Dual:
\[
\label{IKdual}
I_K(\tilde{K}_{\lambda}(;q,t;T;a,b,c,d);q^2,t,T;a,b,c,d)
=
0
\]
unless $\lambda=2\mu$.

Note in fact the nonzero value is foo \comment{add}, which 
can be obtained from a limit of the elliptic case \ref{Rains-to appear}.

\subsubsection{Ideal 2}
\[
S = \langle
T_0T_{2n}^{-1},T_iT_{2n-i}^{-1},T_n\rangle
\]

Functional:
\[
\int
p(q^{1/4} z_1,\dots q^{1/4} z_n,q^{1/4}/z_n,\dots q^{1/4}/z_1)
\Delta_C^{(n)}(\sqrt{t}, -\sqrt{t}, q^{1/4}a, q^{1/4}b; q^{1/2}, t)
%%\dots
\]
($c=q^{1/2}a$, $d=q^{1/2}b$)
$t'=t,q'=q^{1/2},a'=\sqrt{t},b'=-\sqrt{t},c'=q^{1/4}a,d'=q^{1/4}b$

In symmetric function terms,
\[
\label{IK2}
I_K(\tilde{K}_\lambda([p_k(q^{k/2}+q^{-k/2})];q^2,t,T^2;a,b,qa,qb)
   ;q,t,T;\pm\sqrt{t},q^{1/2}a,q^{1/2}b)
=
0
\]
unless $\lambda=\mu^2$.  Dual:
\[
I_K(\tilde{K}_\lambda(;q,t^2;T^2;a,b,ta,tb)
   ;q,t,T;\pm \sqrt{t},a,b)
=
0
\]
unless $\lambda=2\mu$.

